Responsive Parallelism with Futures and State

Motivated by the increasing shift to multicore computers, recent work has developed language support for responsive parallel applications that mix compute-intensive tasks with latency-sensitive, usually interactive, tasks. These developments include calculi that allow assigning priorities to threads, type systems that can rule out priority inversions, and accompanying cost models for predicting responsiveness. These advances share one important limitation: all of this work assumes purely functional programming. This is a significant restriction, because many realistic interactive applications, from games to robots to web servers, use mutable state, e.g., for communication between threads. In this paper, we lift the restriction concerning the use of state. We present $\lambda_i^4$, a calculus with implicit parallelism in the form of prioritized futures and mutable state in the form of references. Because both futures and references are first-class values, $\lambda_i^4$ programs can exhibit complex dependencies, including interaction between threads and with the external world (users, network, etc). To reason about the responsiveness of $\lambda_i^4$ programs, we extend traditional graph-based cost models for parallelism to account for dependencies created via mutable state, and we present a type system to outlaw priority inversions that can lead to unbounded blocking. We show that these techniques are practical by implementing them in C++ and present an empirical evaluation.

==> code-email.tex <==
%\begin{figure}
\begin{lstlisting}[language={[11]C++}]
// pfuture type template: <priority, return-type>
pfuture<SortP, void> *sortF[MAX_USERS];
pfuture<SendP, void> *sendF[MAX_USERS];
pfuture<CompressLoopP, void> *compressLoopF[MAX_USERS];
pfuture<CompressAndPrintP, int> *compressAndPrintF[MAX_USERS][MAX_EMAILS/COMPRESS_CHUNK_SIZE];

template<MyPriority>
void sort(int userID, pfuture<SortP, void> *prevSortF, string sortField) {
  pfuture_touch prevSortF;
  // Sort emails belonging to userID by sortField
}

template<MyPriority>
void send(int userID, pfuture<SendP, void> *prevSendF, Email message) {
  pfuture_touch prevSendF;
  // Send the message
}

template <MyPriority>
int print(int userID, int emailID, pfuture<CompressAndPrintP, int> *thisHandle) {
  int emailChunk = emailID / COMPRESS_CHUNK_SIZE; // integer arithmetic auto floors the value
  pfuture<CompressAndPrintP, int> *prev = ATOMIC_XCHG(&compressAndPrintF[userID][emailChunk], thisHandle);
  if (prev) {
    int compressed = pfut_touch prev;
    if (compressed == COMPRESSED) decompress_chunk(emailChunk);
  }
  printEmail(userID, emailID);
  return DECOMPRESSED;
}

template <MyPriority>
int compress(int emailChunk, pfuture<CompressAndPrintP, int> *thisHandle) {
  pfuture<CompressAndPrintP, int> *prev = ATOMIC_XCHG(&compressAndPrintF[userID][emailChunk], thisHandle);
  int compressed = DECOMPRESSED; // If the handle is NULL, it hasn't been compressed yet
  if (prev) {
    compressed = pfut_touch prev;
  }
  if (compressed == DECOMPRESSED) compress_chunk(emailChunk);
  return COMPRESSED;
}

// Each user connection gets its own email loop which runs at priority LoopP
template<MyPriority>
void per_user_email_loop(int userID, int userSocket) {
  do {
    input = get_input(userSocket); // Get user input
    switch (input.command) {
       case SORT:
          sortF[userID] =
            pfut_create sort<SortP>(userID, sortF[userID], input.sortField);
          break;

       case SEND:
          sendF[userID] =
            pfut_create send<SendP>(userID, sendF[userID], input.message);
          break;

       case PRINT:
          pfuture<CompressAndPrintP, int> *printF = new pfuture<CompressAndPrintP, int>(); 
          // Create the future using the passed in printF handle
          pfut_create<printF> print<CompressAndPrintP>(userID, input.emailID, printF);
    }
  } while (input != DONE);
}

template<MyPriority>
void periodic_compress(int userID) {
  while (!done) {
    nonblocking_sleep(COMPRESS_INTERVAL); // The scheduler can reuse this thread
    // leave the most recent chunk of messages uncompressed
    for (int i = 0; i < email_count(userID)/COMPRESS_CHUNK_SIZE; i++) {
      pfuture<CompressAndPrintP, int> *compressF = new pfuture<CompressAndPrintP, int>();
      pfut_create<compressF> compress<CompressAndPrintP>(userID, i, compressF);
    }
  }
}

template<MyPriority>
int accept_connections_loop() {
  int userID = 0;
  while (!done) {
    int userSocket = accept_user_connection(...);
    pspawn per_user_email_loop<LoopP>(userID, userSocket);
    compressLoopF[userID] = pfuture_create periodic_compress<CompressLoopP>(userID); 
    userID++;
  }
  psync;
  return userID;
}

// main always executes at MyPriority = LowP
int main(int argc, char *argv[]) {
  int maxUserID = pspawn accept_connections_loop<LoopP>();
  psync;

  // Wait for all sorts and sends to complete
  for (int i = 0; i < maxUserID; i++) {
    pfuture_touch sortF[i];
    pfuture_touch sendF[i];
    pfuture_touch compressLoopF[i];
    waitForAllCompressionChunks(compressAndPrintF[userID]);
  }

}

\end{lstlisting}
%\end{figure}


==> code-proxy.tex <==
\begin{lstlisting}[language={[11]C++}]
priority_t LowP, ProxyLogP, ResizeP, WebRequestP, LoopP;

// LoopP > WebRequestP > ResizeP > ProxyLogP > LowP
#pragma priority_decl ProxyLogP > LowP;
#pragma priority_decl WebRequestP > ProxyLogP;
#pragma priority_decl LoopP > WebRequestP;

pfuture<WebRequestP, void> *requestF[MAX_CLIENTS];

template<MyPriority>
void get_website_from_inet(string url, int clientSocket, pfuture<WebRequestP, void> *prev) {
  pfuture_touch prev;
  Website ws = read_from_internet(url); // Actually read from the internet
  send_website_to_client(clientSocket, ws); // Send the website to the requestor
  add_website_to_cache(url, ws); // Add the website to the global website cache
}

// Each client gets its own proxy loop which runs at priority LoopP
template<MyPriority>
void proxy_client_loop(int clientID, int clientSocket) {
  do {
    input = getNetworkInput(clientSocket); // Get user input
    Website *ws = findRequestInCache(input.url);
    if (ws == NULL) { // website not in cache
      requestF[clientID] =
        pfuture_create(WebRequestP, get_website_from_inet, input.url,
                       socket, requestF[clientID]);
    } else {
      send_website_to_client(clientSocket, ws);
    }
  } while (input != DONE);
}

template<MyPriority>
void accept_connections_loop() {
  while (!done) {
    int clientSocket = accept_network_connection(...);
    pspawn proxy_client_loop<LoopP>(clientID, clientSocket);
  }
  psync;
}

template<MyPriority>
void log_statistics_loop() {
  pfuture<ProxyLogP, void> *logF = NULL;
  while(!done) {
    nonblockingSleep(LOGGING_INTERVAL);
    if (logF) pfuture_touch logF;
    logF = pfuture_create collect_and_output_stats<ProxyLogP>();
  }
  if (logF) pfuture_touch logF; // wait for the last logging event
}

int main(int argc, char *argv) {
  pspawn log_statistics_loop<ProxyLogP>();
  pspawn accept_connections_loop<LoopP>();
  psync;

  for (int i = 0; i < MAX_CLIENTS; i++) {
    pfuture_touch requestF[i];
  }
}

\end{lstlisting}
%int main(int argc, char *argv[]) {
%  pfuture<void, LowP> *waitForAll = cilk_pspawn(LoopP, email_loop);
%  cilk_pspawn(CompressP, periodically_compress_emails);
%  cilk_psync;
%
%  pfuture_get(waitForAll);
%
%  return 0;
%}


==> cut.tex <==
%% Impl NEW ------------------------------------------------------------------  

Lastly, a final rule is that, a \code{command} function must either be invoked
using \create  or called within another \code{command} function (with a
special macro, which implicitly inherits the priority of the caller).
Otherwise, in principle, the programmer could do the following:
%
\begin{lstlisting}[language={[11]C++}]
void foo<MyPriority>(arg1, arg2) {
  bar<LowPriority>(arg1, arg2);
}
\end{lstlisting}
%
This is problematic if \code{foo} is invoked with higher priority than
\code{bar}'s low priority, \code{LowPriority}, because we may run into a
priority inversion if another command function \code{quack} with a medium
priority joins with \code{foo}.  Invoking \code{bar} with \create means that
joining with \code{foo} is not blocked by completion of \code{bar}.  The
alternative of calling \code{bar} with a special macro gets around this issue
because \code{bar} is forced to have the same priority as \code{foo}. 

In \calcname{} such an issue does not arise because call is an expression
whereas \create is a command, and therefore the two do not mix.  \ar{Is this
accurate?}  This issue is an artifact of the fact that the distinction between
the command and the expression is not clear in C++.  Nevertheless, our macros
in principle can be implemented as a source-to-source compiler transformation,
and thus with better compiler support, one can check for such a violation at
compile time.\ar{Is this accurate?}

%% Old Impl ------------------------------------------------------------------
%% Type safety stuff

%% Old text % We further cannot guarantee that whenever a future is created
%that the % corresponding thread is executing, because the programmer may
%declare % futures separately from the thread creation. 

%% So long as the programmer only uses our provided API for creating and
%% touching futures, the program compiles using our C++ type system
%% implementation without using unsafe type casts to change the priorities of
%% future handles, and the programmer is careful only to touch futures whose
%% threads are currently executing, then the program will generate only
%% strongly well-formed DAGs.

%% Old Impl ------------------------------------------------------------------

%% TODO: rewrite the discussion about name mangling for the command type
\iffull
The above macros are defined in our implementation in such a way that the
creation of \code{command} functions is opaque to the programmer, and the
actual function names are obfuscated so that they can only be used through
our API functions that ensure they are used safely
\footnote{Technically, this name mangling does not prevent a malicious
  programmer from still calling the underlying command function using a
  standard C++ function call, but we make it more difficult to do accidentally}.
%not be called by the
%programmer accidentally (i.e., we perform name mangling within the macros).
%That is, we explicitly prevent the programmer from \emph{calling} a
%\code{command} function (as opposed to invoking it with \create).
%We forbid
%this because in the \calcname{} a regular function call is an Expression. 
Otherwise, in principle, the programmer could do the following:

%\ksr{Technically, the programmer still can do this. We just make it less obvious
%HOW to do it, so that you have to be quite intentional in your bad behavior
%(i.e. bypassing the API in an obvious way). }

\begin{lstlisting}[language={[11]C++}]
// problematic if MyPriority is instantiated with priority higher than LowPriority
void foo<MyPriority>(arg1, arg2) {
  bar<LowPriority>(arg1, arg2);
}
\end{lstlisting}
%
This is problematic if \code{foo} is invoked with higher priority than
\code{bar}'s low priority, \code{LowPriority}, because we may run into a
priority inversion if later another command function \code{quack} with a
medium priority joins with \code{foo}.

To guarantee safety, a command must either be invoked in a new future
thread using \create, or called from
within another \code{command} function using a special
macro \code{run\_command}, shown below:
%
\begin{lstlisting}[language={[11]C++}]
void foo<MyPriority>(arg1, arg2) {
  run_command(bar, arg1, arg2); // implicitly invoked with MyPriority 
}
\end{lstlisting}
%
%The macro \code{run\_command} takes as the first argument the
%name of the \code{command} function to invoke followed by arguments
%needed by the function. 
Any \code{command} function called in this manner   
implicitly inherits the priority of the calling \code{command} function.
\fi

%% Old Impl ------------------------------------------------------------------

\iffull 
%
To invoke a function with \create to create a future thread, the programmer
uses the following macro:
%
\begin{lstlisting}[language={[11]C++}, firstnumber=last]
// future_pointer = fcreate cmd_name<priority>(args...);
#define create(future_pointer, cmd_name, args...) 
  auto toRun = cmd_name<future_pointer->MyPriority>();
  toRun.runAsFuture(args);
\end{lstlisting}
%
where the \code{cmd_name} is the name of the \code{command} function,
representing the future thread being created, with arguments `\code{args}.'
%Because the future has an associated 
The macro uses the type of the future handle to infer at which priority the
thread needs to run.  Note that this translation means that the
function \code{cmd_name} invoked with \create needs to be a
\code{command} function.  However, \create can
be invoked within any function context, not only within a command.  
%
\fi

Lastly, to ease the declaration of \code{command} functions (classes), we
provide the following macros for declaring a \code{command} function prototype
and for defining a \code{command} function:
%
\begin{lstlisting}[language={[11]C++}]
// prototype / define a command function of the form:
// ReturnType FunctionName(Args...) { FunctionBody }
#define CommandPrototype(ReturnType, FunctionName, Args...);
#define CommandDefine(ReturnType, FunctionName, (Args...), FunctionBody...);
\end{lstlisting}

%
%% Old Impl ------------------------------------------------------------------

This check means that \touch can only be invoked from within a \code{command}
function, and this is the code point where we check that no priority inversion
can occur.% If a priority inversion would occur
%(i.e., \code{this->MyPriority} is not a base class for
%\code{future_pointer->MyPiority}, meaning this thread has higher
%priority than the future thread),
%the static assert would cause a
%compiler error.
%\sr{Changed ``has occurred'' above; that makes it sound more like a dynamic
%  check}

%% Old Impl ------------------------------------------------------------------

In C++, unlike in PriML, the allocation of the future handle and creation of
the associated future thread can be done in two separate steps, i.e.,
allocating the future handle object itself, then invoking \create to form the
association with a future thread.
%\ksr{Async create/touch doesn't feel like the right term; this is really the reference
%polling. An asynchronous (or parallel) create and touch would imply we could
%touch the handle in parallel with the create, which we disallow (unless I am
%mistaken). The create and touch may "appear" to be in parallel, but since there
%is a weak edge they are not. Async allocation/touch?}
%% Old text; I think I got everything
%% In the above pseudocode, when creating a future thread the future is passed in as an
%% argument. Because the future has an associated priority, the macro uses the type
%% of the future to infer at which priority the thread needs to run. 
%% A future can be created either from within regular functions (expressions in
%% \calcname), or from within commands. The \touch, however, can only be executed
%% from within a command because it must be possible to retrieve the priority of
%% the currently executing thread at the time of the \touch. We can ensure there
%% is no priority inversion in the C++ implementation by using a
%% \code{static\_assert} that the priority of the current command
%% (\code{this->MyPriority}) is less than or equal to that of the future's
%% priority (\code{future\_pointer->MyPriority}). If this is not the case, then
%% the current command's priority will not be an ancestor of the future's
%% priority, and the static assert will raise a compiler error.

%% Old Impl ------------------------------------------------------------------

Because we do not have compiler support, we are limited in how clean we can
make the syntax for these macros.
%
When we present pseudocode for example programs, we will show an idealized
syntax specified in a comment above each macro.

\paragraph{Preliminary.} We implemented embodiment of \calcname{} in two
different languages.
%
The first implementation extends Parallel ML and is designed to
faithfully reflect the static and dynamic semantics of \calcname{}.
%
The second implementation is written using C++ templates and extends
Cilk-L, an extension to Cilk (a C/C++-based parallel language) that
includes support for futures and priorities.

The Parallel ML based type system is sound (i.e., there are no false negatives)
and demonstrates that the typing rules described in
Sections~\ref{sec:lang-statics} and \ref{sec:cost} can be implemented
efficiently.  
%
The C++-based implementation is practical and enables us to type check
moderately large Cilk benchmarks that implement interesting functionalities
involving the use of low-level system calls and concurrent data structures
(discussed in \ref{sec:apps}).
%
We leverage the type system of C++ to check the guarantees required by the
typing rules assuming the programmer adheres to a certain programming
discipline.
%
As C++ is not a type-safe language, these checks can be subverted and
it is not possible to provide the same guarantees as in ML.

%% Old Impl ------------------------------------------------------------------

%% As the priority of each task must be retrievable at compile time in order
%to % enforce the typing rules, there are restrictions on which functions can
%use % the \touch Command described in \calcname. These functions must be
%wrapped in % a \code{command class} whose type relies on a template that
%specifies its % execution priority. We simply refer to these functions as
%commands, and they % are analogous to Commands in \calcname. To simplify code
%generation, we % provide macros for defining such commands with a signature
%as follows:

%\ksr{ This is very misleading. Not any function templated with a priority is
%a Command; they must be defined using the CommandPrototype/CommandDefine
%macros.  These classes are (as I understand it) Commands in the calculus. The
%blurry edge is how we use cilk\_run\_command to invoke commands as functions;
%when commands are invoked in this manner, I believe they become expressions
%again. I believe all regular functions (not a command class wrapped function)
%are expressions. } \sr{I found that discussion a little confusing anyway, I
%think it would be clearer to talk about the distinctions between PriML and
%C++ once you've talked about how commands work in C++}

%% Old Impl ------------------------------------------------------------------

\subsection{Parallel ML Implementation}

We have implemented the full type system as an extension of
PriML~\citep{mah-priorities-2018}, which is an extension of Parallel ML with futures and priorities~\citep{spoonhower:phd,rmab-mm-2016,gwraf-hieararchical-2018}.
%
PriML, much like the {\calcname} core calculus, contains an ML-like
expression layer (which, in full PriML, includes most purely functional
features of Standard ML, including algebraic data types, pattern matching,
exceptions, etc.) as well as a command layer that includes operations for
manipulating futures.
%
To this language, we add ML-style mutable references.
%
In the implementation, as in Standard ML, the operations to allocate,
dereference and assign references are part of the expression layer rather
than the command layer.
%
Moving these operations to the expression layer requires no fundamental
changes to the type system.

%% Moving these operations to the expression layer require no fundamental
%% changes to the type system, which is primarily aimed at preventing
%% priority inversions caused by {\touches}.
%% %

The PriML implementation is a compiler front-end, written in Standard ML
and based on the front-end of ML5/pgh~\citep{murphy:phd}.
%
The compiler parses PriML code, including the imperative extensions of this
paper, into an abstract syntax tree.
%
An elaboration pass then converts the abstract syntax tree into an
intermediate language similar to {\calcname}.
%
In the process, it type-checks the code, following rules that quite
closely match those of Section~\ref{sec:lang-statics}.
%
Once the code is determined to be well-typed, the compiler outputs code
in a parallel extension of Standard ML~\citep{spoonhower:phd,rmab-mm-2016,gwraf-hieararchical-2018} by
translating PriML constructs into calls to a threading library built on
top of this parallel ML.

%% \ur{This is redundant.}
%% The addition of references as a built-in construct required extending the
%% syntax and implementing additional typing rules, as well as rules for
%% converting these references into Standard ML references.
%% %
%% No changes were required to the underlying PriML type system---the technical
%% difficulties in adding mutable references to PriML come in the form of
%% modifying the DAG model and cost semantics appropriately to show that
%% mutable state doesn't result in priority inversions (Section~\ref{sec:cost}),
%% rather than in modifying the existing type system.

%\ur{Include some small experiments on the cost of type checking the new language.}

%% Intro ------------------------------------------------------------------

\punt{ We consider two implementations, one extending Parallel ML, which
faithfully encodes the type system, and one built on C++ and Cilk, which can
be used safely with some care. 
%
%% Come back to this
\SYS, following the style of cooperative threading (as traditional
task-parallel platforms do), consists of a runtime scheduler that determines
on-the-fly how to best map logically-parallel computations onto available
processing cores.  Unlike traditional task-parallel platforms, however, it
incorporates mechanisms to support competitive threadings to enable
interactive applications.  Specifically, it supports a programming interface
to allow the programmer to specify the criticality of tasks using priorities.
It has a C++-template-based type system to rule out priority inversions.  The
underlying runtime system automates load balancing while prioritizing
high-priority tasks over lower-priority ones. }

%% Intro ------------------------------------------------------------------

%% \ur{This is just one use of state among many others.  Why discuss this but
%the many others?  % } % Furthermore, in a language with first-class thread
%handles (e.g. of % type~\lstinline{Thread<T>}), the handle to the background
%thread itself % can be stored by reference (e.g. in a global variable of %
%type~\lstinline{Thread<T> *}, using the syntax of C/C++ pointers).  % % %
%This would allow the event loop or another thread to check whether an %
%instance of the background thread has been started.

%% \ur{The next point doesn't seem fundamental. Maybe it is but it is not clear.  Code clarity is usually a surface level issue.  You can have a mostly stupid compiler pass to generate the complex code, can't you.  If there isn't anything fundamental here, I would delagate it to later section, e.g., discussions}

%% The presence of mutable state can sometimes also allow for cleaner code
%% even when all effects are benign.
%% %
%% Consider a dynamic programming algorithm which iteratively fills in the
%% elements of a matrix.
%% %
%% In many such algorithms, the values of the matrix elements depend on each other
%% in such a way that many, but not all, elements can be computed in parallel.
%% %
%% This can be encoded in a cooperatively parallel system using one thread for
%% each matrix element, where the dependency structure of the threads mirrors that
%% of the matrix elements.
%% %
%% In a functional implementation, the function to compute a particular element
%% must take as arguments all of the elements on which it might depend.
%% %
%% For example:
%% \begin{lstlisting}[numbers=none, language=ML]
%% fun computeElement(e1 : T thread, ..., en : T thread) : T =
%%   f(get e1, ..., get en)
%% \end{lstlisting}
%% %
%% This can quickly result in complex code because each function must
%% take many arguments, and we may even need several versions of the
%% function with different numbers of arguments (e.g., if the first row
%% of the matrix doesn't depend on other elements).
%% %
%% In an imperative implementation, we can simply declare an array of thread
%% handle references and spawn the functions iteratively.
%% \begin{lstlisting}[numbers=none]
%% Thread<T> *mat[M][N];
%% void computeElement(int x, int y) {
%%   // suppose element (x, y) depends on (x0, y0), ..., (xn, yn)
%%   return f(mat[x0][y0]->get(), ..., mat[xn][yn]->get())
%% }
%% \end{lstlisting}


%% App ------------------------------------------------------------------

\subsection{Proxy Server} \label{sec:apps_proxy}

Our first case study is a proxy server that allows multiple clients to connect
and request websites by their URL. The server then fetches the
corresponding website on the client's behalf, masking the client's IP address.
As an optimization, the server
maintains a cache of website contents represented as a concurrent hashtable.
If a website is in the
cache, the server can respond with it immediately.
%
\iffull
This case study is of interest because it relies on system-level socket
programming to handle network connections, requires code to deal with network
connection errors, and makes heavy use of a concurrent hashtable to cache
websites requested by clients.
\fi

The application itself utilizes four different priority levels.  Both the loop
that accepts client connections and the per-client event loop that handles the
client requests are serviced at the highest priority, \code{LoopP}, in order
to accept connections and service requests as quickly as possible.  If the
proxy server needs to fetch a website from the world-wide web, the fetch
operation runs at the next highest priority, \code{WebReqP}, so the client
does not wait for long for the website content.  Logging statistics is not an
interactive activity, and thus runs at the second lowest priority,
\code{ProxyLogP}.  To be able to synchronize with all other threads,
\code{main} runs at the lowest priority, \code{LowP}.

\iffull
The following pseudocode represents the priorities used by the application, as
well as the global future references used and the signatures for commands that
provide the outlined functionality:\footnote{In all pseudocode shown, we
utilize the idealized syntax discussed in \secref{impl}.}

\begin{lstlisting}[language={[11]C++}]
priority_t LowP, ProxyLogP, WebReqP, LoopP;
#pragma priority_decl LoopP > WebReqP > ProxyLogP > LowP;

future<WebReqP, void> *reqF[MAX_CLIENTS];
template<class MyPriority = ProxyLogP> void log_statistics(); 
template<class MyPriority = LoopP> int accept_connections(); 
template <class MyPriority = LoopP> void client_loop(int clientID, int clientSocket); 
template <class MyPriority = WebReqP> 
    void fetch_website(string url, int clientSocket, future<WebReqP, void> *prev); 
\end{lstlisting}
%
\else
The following pseudocode represents the priorities used by the 
application.\footnote{In all pseudocode shown, we
utilize the idealized syntax discussed in \secref{impl}.}

\begin{lstlisting}[language={[11]C++}]
priority_t LowP, ProxyLogP, WebReqP, LoopP;
#pragma priority_decl LoopP > WebReqP > ProxyLogP > LowP;
\end{lstlisting}
\fi

By default the entry point of the program (i.e., user-defined \code{main}
function) has the lowest priority \code{LowP},\footnote{This is accomplished 
by the system providing a separate \code{main} function and renaming the
user-defined \code{main} and wrapping it with the \code{CommandDefine}
discussed in \secref{impl}.} Its implementation is shown below: 
%
\begin{lstlisting}[language={[11]C++}]
int main(int argc, char *argv) {
  future<LoopP, int> *acceptF = @\create{}@ accept_connections<LoopP>();
  future<ProxyLogP, void> *logF = @\create{}@ log_statistics<ProxyLogP>();
  @\touch{}@ logF;
  int totalConnections = @\touch{}@ acceptF;
  for (int i = 0; i < totalConnections; i++) { @\touch{}@ reqF[i]; }
}
\end{lstlisting}
 
The \code{main} function creates a future thread to handle accepting new
client connections with \code{accept\_connections} and then another future
thread to handle logging statistics about the server's usage.  It then touches
both of these futures to wait until they complete (which occurs when the
server is being shut down), after which it touches all of the valid
\code{reqF} references to ensure all outstanding future threads created to
fetch websites complete before exiting.  The use of
future handle references in the nonlocal array \code{reqF} allows for
cleaner code, as the future handle references stored in this array are
produced by \code{client_loop}, which is multiple call-chain levels away
from \code{main}.  Using \code{reqF} for such a purpose prevents proliferation
of arguments and return values.

\iffull
\begin{lstlisting}[firstnumber=last,language={[11]C++}]
int accept_connections() {
  int clientID = 0;
  future<LoopP, void> *loopF[MAX_CLIENTS];
  while (!done) {
    int clientSocket = accept_user_connection(...);
    loopF[clientID++] = @\create{}@ client_loop<LoopP>(clientID, clientSocket);
  }
  // ensure all connections terminate before returning
  for (int i=0; i < clientID; i++) { @\touch{}@ loopF[i]; }
  return clientID; // return total number of connections
}
\end{lstlisting}

The \code{accept\_connections} future thread created by \code{main} invokes 
\code{accept_user_connection}, which implicitly (not shown) uses  
latency-hiding futures to accept new client connections, which does not return
until a connection is made.  Upon returning, it creates a future thread to handle 
the new client's requests using \code{client_loop}.  Note that requests from 
multiple clients are handled in parallel as \code{client_loop} is invoked using
\create. 

Within the \code{log_statistics} command, a latency-hiding operation is
used to sleep for a predefined interval, after which the command collects and
outputs statistics to a log by creating a future thread. If such a thread has
previously been created, the command will touch the associated future before
creating the next future thread for logging.

In the \code{client_loop} command, the proxy server again uses latency-hiding
futures to receive requests for URLs from the client (in
\code{get_network_input}).  The proxy server then checks a concurrent
hashtable, which serves as a cache that holds previously requested websites,
to see if the particular URL has been requested.  If the website is found in
the cache, it is immediately sent back to the client. If not, the
\code{client_loop} creates a new future thread to run the \code{fetch_website}
command to get the website from the internet. 

% As the \code{client_loop} is a fairly straightforward loop
% that merely responds to events, it would be straightforward to create an
% interface for true event-driven programming by allowing users to specify a
% Command callback for specific events.

\begin{lstlisting}[firstnumber=last,language={[11]C++}]
void client_loop(int clientID, int clientSocket) {
  do {
    input = get_network_input(clientSocket); // Get user input
    Website *ws = find_website_in_cache(input.url);
    if (ws == NULL) { // website not in cache
      reqF[clientID] = @\create{}@ fetch_website<WebReqP>(input.url, socket, reqF[clientID]);
    } else {
      send_website_to_client(clientSocket, ws);
    }
  } while (input != DONE);
}
\end{lstlisting}
%
\else
Due to space constraints, we omit details of most functions, but we will walk
through the event loop that handles a single client's request:
%
\begin{lstlisting}[firstnumber=last,language={[11]C++}]
void client_loop(int clientID, int clientSocket) {
  do {
    input = get_network_input(clientSocket); // Get user input
    Website *ws = find_website_in_cache(input.url);
    if (ws == NULL) { // website not in cache
      reqF[clientID] = @\create{}@ fetch_website<WebReqP>(input.url, socket, reqF[clientID]);
    } else {
      send_website_to_client(clientSocket, ws);
    }
  } while (input != DONE);
}
\end{lstlisting}
%
The \code{client_loop} command is created to handle a single client connection.  
The proxy server again uses latency-hiding futures to receive requests for
URLs from the client (in \code{get_network_input}).  The proxy server then
checks a concurrent hashtable, which serves as a cache that holds previously
requested websites. If the website is found in the cache, it is immediately
sent back to the client. If not, \code{client_loop} creates a new future
thread to run \code{fetch_website}, which requests the website using HTTP.
We want to limit each client to one outstanding HTTP request.
Thus, \code{fetch_website} touches the handle
from the previous request (passed in as the 3rd argument) before beginning
the next request.  At the end of the computation,
\code{reqF[clientID]} stores the future reference for the last outstanding
request from the client, which is touched in \code{main}, as shown
earlier. 
\fi %%%%%%%%%%%%% END OF IF FULL

\iffull
Within the \code{fetch_website} function, the previous request by
this client is touched to restrict each user to one outstanding HTTP request.
The server then loads the website from the internet on behalf of the client, and
sends the received website to the client. The implementation of these two
functions is as follows:
%
\begin{lstlisting}[firstnumber=last,language={[11]C++}]
void fetch_website(string url, int clientSocket,
                   future<WebReqP, void> *prev) {
  @\touch{}@ prev;
  Website *ws = read_from_internet(url); // Actually read from the internet
  send_website_to_client(clientSocket, ws); // Send the website to the requester
  add_website_to_cache(url, ws); // Add the website to the global website cache
}
\end{lstlisting}

At the end of the computation,
\code{reqF[clientID]} stores the future handle for the last outstanding
request from the client, which is then touched in \code{main}, as shown 
earlier.
\fi  %%%%%%%%%%%% END OF IF FULL

\iffull %%%%%%%%%%%% BEGIN IF FULL
\else
The proxy server implementation, both with and without the
priority annotations, comes in at around 1100 lines of code.
In three compilations of each, the maximum compilation time was 4.39 seconds
with the priority encoding and 3.09 seconds without.
\fi %%%%%%%%%%%% END OF IF FULL

%\input{code-proxy.tex}

%% ----------------------------------------------
%% Macros for notes
\newif\ifnotes
% Options
\DeclareOption{notes}{\notestrue}
\DeclareOption{nonotes}{\notesfalse}
\ExecuteOptions{notes}
\ProcessOptions\relax

\notestrue

\newcommand{\cnote}[2]{%
  \ifnotes%
    {[[{\color{#1}\scriptsize \sf \raggedright{#2}}]]}%
  \fi}

\newcommand{\anote}[1]{\cnote{red}{Ange: #1}}
\newcommand{\unote}[1]{\cnote{blue}{Umut: #1}}
\newcommand{\snote}[1]{\cnote{purple}{Stefan: #1}}
\newcommand{\knote}[1]{\cnote{brown}{Kyle: #1}}



==> fig-cost.tex <==
\begin{figure*}
\langfigsize
    \centering
  \def \MathparLineskip {\lineskip=\mylineskip}
\begin{mathpar}
\Rule{C-Val}
      {\strut}
      {\ceval[\dassn]{v}{v}{\ethread}}
\and
\Rule{C-Let}
      {\ceval[\dassn]{e_1}{v_1}{\uthread_1}\\
        \ceval[\dassn]{[v_1/x]e_2}{v}{\uthread_2}\\
        u\fresh}
      {\ceval[\dassn]{\kwlet{x}{e_1}{e_2}}{v}
        {\uthread_1 \tscomp{} u \tscomp{} \uthread_2}}
\and
\Rule{C-Ifz-NZ}
      {\ceval[\dassn]{[\kwnumeral{n}/x]e_2}{v}{\uthread}\\
        u \fresh}
      {\ceval[\dassn]{\kwifz{\kwnumeral{n+1}}{e_1}{x}{e_2}}{v}
        {u \tscomp{} \uthread}}
\and
\Rule{C-Ifz-Z}
      {\ceval[\dassn]{e_1}{v}{\uthread}\\
        u \fresh}
      {\ceval[\dassn]{\kwifz{\kwnumeral{0}}{e_1}{x}{e_2}}{v}
        {u \tscomp{} \uthread}}
\and
\Rule{C-App}
      {\ceval[\dassn]{[v/x]e}{v'}{\uthread}\\
        u \fresh}
      {\ceval[\dassn]{\kwapply{(\kwfun{x}{e})}{v}}{v'}
        {u \tscomp{} \uthread}}
\and
\Rule{C-PiApp}
     {\ceval[\dassn]{[\kwn/x]e}{v'}{\uthread}\\
       u \fresh}
     {\ceval[\dassn]{\kwproj{\kwarray{x}{e}}{\kwn}}{v'}
       {u \tscomp{} \uthread}}
\and
%% \Rule{C-Pair}
%%       {u \fresh}
%%       {\ceval[\dassn]{\kwepair{v_1}{v_2}}{\kwpair{v_1}{v_2}}
%%         {u}}
%% \and
\Rule{C-Fst}
      {u \fresh}
      {\ceval[\dassn]{\kwfst{\kwepair{v_1}{v_2}}}{v_1}{u}}
\and
\Rule{C-Snd}
      {u \fresh}
      {\ceval[\dassn]{\kwsnd{\kwpair{v_1}{v_2}}}{v_2}{u}}
\and
%% \Rule{C-InL}
%%       {u \fresh}
%%       {\ceval[\dassn]{\kweinl{v}}{\kwinl{v}}{u}}
%% \and
%% \Rule{C-InR}
%%       {u \fresh}
%%       {\ceval[\dassn]{\kweinr{v}}{\kwinr{v}}{u}}
%% \and
\Rule{C-Case-L}
      {\ceval[\dassn]{[v/x]e_1}{v'}{\uthread}\\
        u \fresh}
      {\ceval[\dassn]{\kwcase{\kweinl{v}}{x}{e_1}{y}{e_2}}{v'}
        {u \tscomp{} \uthread}}
\and
\Rule{C-Case-R}
      {\ceval[\dassn]{[v/y]e_2}{v'}{\uthread}\\
        u \fresh}
      {\ceval[\dassn]{\kwcase{\kweinr{v}}{x}{e_1}{y}{e_2}}{v'}
        {u \tscomp{} \uthread}}
\and
%% \Rule{C-Output}
%%       {u \fresh}
%%       {\ceval[\dassn]{\kwoutput{v}}{\kwtriv}{u}}
%% \and
%% \Rule{C-Input}
%%       {%u_1, u_2 \fresh\\
%%         u\fresh
%%         %\dassn(\dvar) = \delay
%%       }
%%       {\ceval[\dassn]{\kwinput}{\kwn}
%%         %{u_1 \tscomp{\delay} u_2}}
%%         {u}}
%% \and
\Rule{C-TApp}
      {\ceval[\dassn]{[a/\thvar]e}{v}{\uthread}\\
        u \fresh}
      {\ceval[\dassn]{\kwapply{(\kwwlam{\thvar}{\cons}{e})}{a}}{v}
        {u \tscomp{} \uthread}}
\and
\Rule{C-Fix}
      {\ceval[\dassn]{[v/x]e}{v'}{\uthread}\\
        u \fresh}
      {\ceval[\dassn]{\kwfix{x}{\tau}{e}}{v'}{u \tscomp{} \uthread}}
\end{mathpar}
%
\begin{mathpar}
\Rule{C-Bind}
      {\ceval[\dassn]{e}{\kwcmd{\prio}{\cmd_1}}{\uthread_1}\\
        \cceval{\tsig}{\sig}{a}{\prio}{\cmd_1}{v}{\graph_1}{\tsig_1}{\sig_1}\\
        u \fresh\\
        \cceval{\tsig_1}{\sig_1}{a}{\prio}{[v/x]\cmd_2}{v'}{\graph_2}{\tsig_2}{\sig_2}\\
        }
      {\cceval{\tsig}{\sig}{a}{\prio}{\kwbind{e}{x}{\cmd_2}}{v'}
        {\sgraph{\uthread_1} \scomp{a}
          \graph_1 \scomp{a} \sgraph{u} \scomp{a} \graph_2}{\tsig_2}{\sig_2}
      }
\and
\Rule{C-Spawn}
     {\ceval[\dassn]{e}{\kwtid{b}}{\uthread}\\
        \cceval{\tsig}{\sig}{b}{\prio'}{\cmd}{v}
               {\dagq{\dthreads}{\spawns}{\syncs}{\polls}}
               {\tsig,\tsig'}{\sig,\sig'}\\
        u \fresh
        }
      {\cceval{\tsig}{\sig}{a}{\prio}
        {\kwbspawn{e}{\cmd}}{\kwtriv}
        {\dagq{\cthread{a}{\prio}{\uthread \tscomp{} u} \uplus \dthreads}
          {\spawns \cup \{(u, b)\}}{\syncs}{\polls}}
        {\tsig,\tsig',\sigcent{b}{v}{\sig'}}
        {\sig,\sigtype{b}{\tau}{\prio'}}
      }
\and
\Rule{C-Sync}
      {\ceval[\dassn]{e}{\kwtid{b}}{\uthread}\\
        u \fresh}
      {\cceval{\tsig,\sigcent{b}{v}{\sig'}}
        {\sig,\sigtype{b}{\tau}{\prio'}}{a}{\prio}
        {\kwbsync{e}}
        {v}
        {\dagq{\cthread{a}{\prio}{\uthread \tscomp{} u}}{\emptyset}
          {\{(b, u)\}}{\emptyset}}{\tsig,\sigcent{b}{v}{\sig'}}{\sig,\sigtype{b}{\tau}{\prio'}, \sig'}
      }
%% \and
%% \Rule{C-Poll-Some}
%%       {u \fresh}
%%       {\cceval{a}{\prio}
%%         {\kwpoll{\kwtd{b}{v}}}
%%         {\kwinl{v}}
%%         {\dagq{\cthread{a}{u}}{\emptyset}{\emptyset}{\{(b, u)\}}}}
%% \and
%% \Rule{C-Poll-None}
%%       {u \fresh}
%%       {\cceval{a}{\prio}
%%         {\kwpoll{\kwtd{b}{v}}}
%%         {\kwinr{\kwtriv}}
%%         {\dagq{\cthread{a}{u}}{\emptyset}{\emptyset}{\emptyset}}}
%%         {\dagq{\dthreads}{\spawns}{\syncs}{\polls}}}
\and
\Rule{C-Ret}
      {\ceval[\dassn]{e}{v}{\uthread}}
      {\cceval{\tsig}{\sig}{a}{\prio}{\kwret{e}}{v}
        {\dagq{\cthread{a}{\prio}{\uthread}}{\emptyset}{\emptyset}{\emptyset}}
        {\tsig}{\sig}
      }
\end{mathpar}
\caption{Cost semantics}
\label{fig:cost}
\end{figure*}

